New Facts and Data about Professors and their Research

We introduce a new survey of professors at roughly 150 of the most research-intensive institutions of higher education in the US. We document seven new features of how research-active professors are compensated, how they spend their time, and how they perceive their research pursuits: (1) there is more inequality in earnings within fields than there is across fields; (2) institutions, ranks, tasks, and sources of earnings can account for roughly half of the total variation in earnings; (3) there is significant variation across fields in the correlations between earnings and different kinds of research output, but these account for a small amount of earnings variation; (4) measuring professors' productivity in terms of output-per-year versus output-per-research-hour can yield substantial differences; (5) professors' beliefs about the riskiness of their research are best predicted by their fundraising intensity, their risk-aversion in their personal lives, and the degree to which their research involves generating new hypotheses; (6) older and younger professors have very different research outputs and time allocations, but their intended audiences are quite similar; (7) personal risk-taking is highly predictive of professors' orientation towards applied, commercially-relevant research.

==> figtab/stub_tasksposttenure_note1.tex <==
In the first ten years post tenure, approximately 80\% of the decline in research and fundraising efforts can be explained by the increase in teaching, administrative, and other efforts.


==> figtab/tab_pwcorr_hrshr_uncond_fullsamp.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
                &\multicolumn{6}{c}{}                                                                                             \\
                & research         &fundraising         & teaching         &administ.         & clinical         &    other         \\
\hline
research        &     1         &                  &                  &                  &                  &                  \\
fundraising     &    --0.09\sym{***}&     1         &                  &                  &                  &                  \\
teaching        &    --0.44\sym{***}&    --0.25\sym{***}&     1         &                  &                  &                  \\
administ.       &    --0.45\sym{***}&    --0.15\sym{***}&    --0.03\sym{*}  &     1         &                  &                  \\
clinical        &    --0.30\sym{***}&    --0.18\sym{***}&    --0.22\sym{***}&    --0.10\sym{***}&     1         &                  \\
other           &    --0.19\sym{***}&    --0.06\sym{***}&    --0.09\sym{***}&    --0.12\sym{***}&    --0.10\sym{***}&     1         \\
\hline\hline
\end{tabular}
}

